PolyChaos.jl -- A Julia Package for Polynomial Chaos in Systems and Control

Polynomial chaos expansion (PCE) is an increasingly popular technique for uncertainty propagation and quantification in systems and control. Based on the theory of Hilbert spaces and orthogonal polynomials, PCE allows for a unifying mathematical framework to study systems under arbitrary uncertainties of finite variance; we introduce this problem as a so-called mapping under uncertainty. For practical PCE-based applications we require orthogonal polynomials relative to given probability densities, and their quadrature rules. With PolyChaos we provide a Julia software package that delivers the desired functionality: given a probability density function, PolyChaos offers several numerical routines to construct the respective orthogonal polynomials, and the quadrature rules together with tensorized scalar products. PolyChaos is the first PCE-related software written in Julia, a scientific programming language that combines the readability of scripted languages with the speed of compiled languages. We provide illustrating numerical examples that show both PCE and PolyChaos in action.

==> macros/abbreviations.tex <==
\newcommand{\problemautorefname}{Problem\xspace}
\newcommand{\assautorefname}{Assumption\xspace}
\newcommand{\defiautorefname}{Definition\xspace}
\newcommand{\thmautorefname}{Theorem\xspace}
\newcommand{\coroautorefname}{Corollary\xspace}
\newcommand{\propautorefname}{Proposition\xspace}
\newcommand{\lemmautorefname}{Lemma\xspace}
\newcommand{\statautorefname}{Statement\xspace}
\newcommand{\remaautorefname}{Remark\xspace}
\newcommand{\conjautorefname}{Conjecture\xspace}
\newcommand{\exmplautorefname}{Example\xspace}
\newcommand{\settautorefname}{Setting\xspace}

% Abbreviations
\usepackage[acronym,nonumberlist,nopostdot,toc]{glossaries}
\setglossarystyle{long}
\renewenvironment{theglossary}%
{\begin{longtable}[l]{ll}}%
	{\end{longtable}}
\makeglossaries
\newacronym{pce}{\textsc{pce}}{polynomial chaos expansion}
\newacronym{pdf}{\textsc{pdf}}{probability density function}
\newacronym{opf}{\textsc{opf}}{optimal power flow}
\newacronym{pf}{\textsc{pf}}{power flow}
\newacronym{ppf}{\textsc{ppf}}{probabilistic power flow}
\newacronym{ccopf}{\textsc{cc}-\textsc{opf}}{chance-constrained optimal power flow}
\newacronym{bfs}{\textsc{bfs}}{backward-forward sweep}
\newacronym{dc}{\textsc{dc}}{direct current}
\newacronym{ac}{\textsc{ac}}{alternating current}
\newacronym{ptdf}{\textsc{ptdf}}{power transfer distribution factor}
\newacronym{nlp}{\textsc{nlp}}{nonlinear program}
\newacronym{kl}{\textsc{kl}}{Karhunen-Lo\`eve}
\newacronym{cc}{\textsc{cc}}{chance constraint}
\newacronym{qp}{\textsc{qp}}{quadratic program}
\newacronym{socp}{\textsc{socp}}{second-order cone program}
\newacronym{mpc}{\textsc{mpc}}{model predictive control}
\newacronym{lti}{\textsc{lti}}{linear time-invariant}
\newacronym{kkt}{\textsc{kkt}}{Karush Kuhn Tucker}
\newacronym{mc}{\textsc{mc}}{Monte-Carlo}
\newacronym{licq}{\textsc{licq}}{linear inequality constraint qualification}
\newacronym{eeg}{\textsc{eeg}}{Erneuerbare-Energien-Gesetz}
\newacronym{dry}{\textsc{dry}}{Don't Repeat Yourself}
\newacronym{wet}{\textsc{wet}}{Write Everything Twice}

\newcommand{\lu}{\textsc{lu}\xspace}
\newcommand{\pdf}{\gls{pdf}\xspace}
\newcommand{\pdfs}{\glspl{pdf}\xspace}
\newcommand{\opf}{\gls{opf}\xspace}
\newcommand{\pf}{\gls{pf}\xspace}
\newcommand{\ppf}{\gls{ppf}\xspace}
\newcommand{\bfs}{\gls{bfs}\xspace}
\newcommand{\DC}{\gls{dc}\xspace}
\newcommand{\AC}{\gls{ac}\xspace}
%\newcommand{\acopf}{\AC-\opf\xspace}
%\newcommand{\dcopf}{\DC-\opf\xspace}
\newcommand{\ptdf}{\gls{ptdf}\xspace}
\newcommand{\acptdf}{\AC-\ptdf\xspace}
\newcommand{\nlp}{\gls{nlp}\xspace}

\newcommand{\pce}{\gls{pce}\xspace}
\newcommand{\pces}{\glspl{pce}\xspace}
\newcommand{\kl}{\gls{kl}\xspace}


\newcommand{\cc}{\gls{cc}\xspace}
\newcommand{\ccs}{\glspl{cc}\xspace}
\newcommand{\ccopf}{\gls{ccopf}\xspace}

\newcommand{\qp}{\gls{qp}\xspace}
\newcommand{\qps}{\glspl{qp}\xspace}
\newcommand{\socp}{\gls{socp}\xspace}
\newcommand{\socps}{\glspl{socp}\xspace}
\newcommand{\mpc}{\gls{mpc}\xspace}
\newcommand{\lti}{\gls{lti}\xspace}
\newcommand{\eeg}{\gls{eeg}\xspace}
\newcommand{\dry}{\gls{dry}\xspace}
\newcommand{\wet}{\gls{wet}\xspace}


\newcommand{\Nx}{n_{\chi}}
\newcommand{\Ncon}{n_{\text{\normalfont con}}}
\newcommand{\Nact}{n_{\text{\normalfont act}}}
\newcommand{\licq}{\gls{licq}\xspace}
\newcommand{\Aact}{A_{\text{\normalfont act}}}
\newcommand{\Mact}{M_{\mathcal{A}}}
\newcommand{\argmin}[1]{\underset{#1}{\operatorname{argmin~}}}

\newcommand{\kkt}{\gls{kkt}\xspace}

\newcommand{\mc}{\gls{mc}\xspace}

\newcommand{\polychaos}{\code{PolyChaos.jl}\xspace}

\newcommand{\aeligature}{\ae\xspace}

